Falcon: Accelerating Homomorphically Encrypted Convolutions for Efficient Private Mobile Network Inference

Efficient networks, e.g., MobileNetV2, EfficientNet, etc, achieves state-of-the-art (SOTA) accuracy with lightweight computation. However, existing homomorphic encryption (HE)-based two-party computation (2PC) frameworks are not optimized for these networks and suffer from a high inference overhead. We observe the inefficiency mainly comes from the packing algorithm, which ignores the computation characteristics and the communication bottleneck of homomorphically encrypted depthwise convolutions. Therefore, in this paper, we propose Falcon, an effective dense packing algorithm for HE-based 2PC frameworks. Falcon features a zero-aware greedy packing algorithm and a communication-aware operator tiling strategy to improve the packing density for depthwise convolutions. Compared to SOTA HE-based 2PC frameworks, e.g., CrypTFlow2, Iron and Cheetah, Falcon achieves more than 15.6x, 5.1x and 1.8x latency reduction, respectively, at operator level. Meanwhile, at network level, Falcon allows for 1.4% and 4.2% accuracy improvement over Cheetah on CIFAR-100 and TinyImagenet datasets with iso-communication, respecitvely.

==> doc/abandon.tex <==
Now, we present our complete protocol for depth-wise convolution.

\begin{algorithm}[h]
\DontPrintSemicolon
  \SetAlgoLined
  \KwIn {Client holds $ \langle \textbf{X} \rangle^C \in\mathbb{Z}^{H\times W\times C}_{2^l}$, and Server holds both $\langle \textbf{X} \rangle^S\in\mathbb{Z}^{H\times W\times C}_{2^l}$ and $\textbf{W}\in \mathbb{Z}^{h\times h\times C}_{2^l}$.}
  \KwOut {Client and Server get $\langle \textbf{Y} \rangle^C,\langle \textbf{Y} \rangle^S \in\mathbb{Z}^{H'\times W'\times C}$, respectively, where $\textbf{Y}=\text{DWConv}(\textbf{X},\textbf{W})$.}
  Client, Server compute the partition window size $C_x,C_w$ such that meets equation (\ref{eq:target}) (\ref{eq:constraint1}) (\ref{eq:constraint2}). Let $n_{x}=\lceil C/C_x\rceil$, and $n_{w}=\lceil C/C_w\rceil$.\;
  
  Client partitions its share tensor into sub-blocks $\langle \textbf{X}_c \rangle^C \in\mathbb{Z}^{H\times W\times C_x}_{2^l}$, for $c \in [n_x]$.\;
  
  Client then encodes the sub-blocks as polynomials $\langle \hat{x}_c \rangle^C=\pi_{\mathrm{dwconv}}^i(\langle \textbf{X}_c \rangle^C) $ and 
 sends the ciphertext $\mathrm{CT}=\operatorname{Enc}(\langle \hat{x}_c \rangle^C)$ to Server.\;
  
  Server partitions its weight tensor into sub-blocks $ \textbf{W}_{c^{\prime}}  \in\mathbb{Z}^{h\times h\times C_w}_{2^l}$, for $c^{\prime} \in [n_w]$.\;
  
  Server encodes its share of input tensor and the filter as polynomials$\langle \hat{x}_{c} \rangle^S=\pi_{\mathrm{dwconv}}^i(\langle \textbf{X}_{c} \rangle^S), \hat{w}_{c^{\prime}} =\pi_{\mathrm{conv}}^w( \textbf{W}_{c^{\prime}} )$.\;
  
  Server samples $\textbf{R}\in\mathbb{Z}^{ H^{\prime}\times W^{\prime}\times C}_{2^l}$ uniformly at random.\;
  
  On receing the RLWE ciphertext $\mathrm{CT}$ from Client, Server operates to obtain $\mathrm{CT}^\prime=(\mathrm{CT}\boxplus\langle \hat{x}_{c} \rangle^S)\boxtimes \hat{w}_{c^{\prime}}$ for  $c \in [n_x],c^{\prime} \in [n_w]$.\;

  \textbf{[Extract and Re-mask]}. For each $i^\prime \in [H^\prime],j^\prime \in [W^\prime],k^\prime \in [C]$, Server first extracts a LWE ciphertext $\mathrm{ct}_{i^\prime,j^\prime,k^\prime}=\operatorname{Extract}(\mathrm{CT}^\prime,(Sh(k^\prime)+k^\prime)*H*W+\mathrm{O}+i^{\prime} s W+j^{\prime} s)$ and then re-masks it via $\mathrm{ct}^\prime_{i^\prime,j^\prime,k^\prime}=\mathrm{ct}_{i^\prime,j^\prime,k^\prime}\boxminus \textbf{R}[i^\prime,j^\prime,k^\prime]$. Server then sends the ciphertexts {$\mathrm{ct}^\prime_{i^\prime,j^\prime,k^\prime}$} back to Client\;
  
  Server outputs $\textbf{R}$ mod $2^l$ as the share $\langle \textbf{Y} \rangle^S$.\;
  On receiving the LWE ciphertexts from Server, Client computes $\langle \textbf{Y} \rangle^C[i^\prime,j^\prime,k^\prime]=\operatorname{Dec}(\mathrm{ct}^\prime_{i^\prime,j^\prime,k^\prime})$ for all positions ($i^\prime,j^\prime,k^\prime$).\;
  
  
  \caption{Secure Depth-wise Convolution Protocol}
\end{algorithm}

\begin{table*}[!tb]
\caption{depth-wise conv under different N}
\begin{center}
\resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{N}}
     & \multicolumn{2}{|c|}{\textbf{CrypTFlow2}}& \multicolumn{2}{|c|}{\textbf{Iron}}& \multicolumn{2}{|c|}{\textbf{Cheetah}}& \multicolumn{2}{|c|}{\textbf{GP}}& \multicolumn{2}{|c|}{\textbf{GP+tile}}\\
    \cline{2-11}
    & Comm.(MB)  & Latency(s) &  Comm.(MB)  & Latency(s) & Comm.(MB)  & Latency(s) & Comm.(MB)  & Latency(s) & Comm.(MB)  & Latency(s)\\
    \hline
    4096& 9.00  &26.57&51.70&6.79&18.94&3.46&10.77&1.77&8.98&1.58\\
    \hline
    8192& 18.00&52.32&102.69&13.22&35.77&6.02&19.12&3.64&13.21&2.76\\
    \hline
    16384& 36.00&107.15&204.14&34.03&70.10&11.63&34.47&7.05&17.45&4.31\\
    \hline
    32768& 72.00&210.24&409.35&77.28&140.16&23.86&71.26&13.58&26.04&7.28\\
    \hline
    \end{tabular}
}
\label{tab:impact_dim}
\end{center}
\end{table*}

\begin{table*}[h]
\caption{depth-wise conv under different dimensions(the dimensions are represented by activation resolution, channels, and kernel size)}
\begin{center}
\resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{Conv dim}}
     & \multicolumn{2}{|c|}{\textbf{CrypTFlow2}}& \multicolumn{2}{|c|}{\textbf{Iron}}& \multicolumn{2}{|c|}{\textbf{Cheetah}}& \multicolumn{2}{|c|}{\textbf{GP}}& \multicolumn{2}{|c|}{\textbf{GP+tile}}\\
    \cline{2-11}
    & Comm.(MB)  & Latency(s) &  Comm.(MB)  & Latency(s) & Comm.(MB)  & Latency(s) & Comm.(MB)  & Latency(s) & Comm.(MB)  & Latency(s)\\
    \hline
    (28,192,3)& 12.01  & 12.13 & 23.50 &4.00& 8.71&1.27&6.45&0.76&6.45&0.72\\
    \hline
    (14,384,3)& 6.00  & 13.88 &34.46&4.54&12.66&1.98&7.22&1.21&5.99&0.89\\
    \hline
    (14,576,3)& 9.00&26.57&51.70&6.80&18.94&2.97&10.77&1.82&8.98&1.37\\
    \hline
    (7,960,3)&4.00&30.39&85.29&10.35&28.66&5.55&14.76&2.71&7.23&1.73\\
    \hline
    \end{tabular}
}
\label{tab:impact_dim}
\end{center}
\end{table*}

 Formally, the coefficient mapping for input remains the same as before, while the mapping for weights, denoted as $\pi_{\mathrm{gconv}}^w:\mathbb{Z}^{C_w^\prime\times G \times G\times R\times R}_p\longmapsto \mathbb{A}_{N,p}$, is as follows:
\begin{align}
    \hat{w}=\pi_{\mathrm{gconv}}^w(\mbm{W})\text { st. }\hat{w} [\offset(c^\prime)\times HWG^2+O \notag\\
    -g_1^\prime HWG-g_2^\prime HW-lW-l^{\prime}]=\mbm{W}[c^\prime,g_1^\prime,g_2^\prime,l,l^{\prime}] 
\end{align}
where $O=HW(G^2-1)+W(h-1)+h-1$ and $\offset$ is:
\begin{equation}
    \offset(c^{\prime})=\left\{\begin{array}{l}
\left(C_x+2\right) *\left(C_w-1-c^\prime\right), c^\prime \geqslant \frac{C_w^\prime}{2} \\
C_x+c^\prime*\left(C_x+1\right), c^\prime<\frac{C_w^\prime}{2}
\end{array}\right.
\end{equation}
For the output, we reshape it into dimensions of $n_g\times G\times H^\prime \times W^\prime$. Then, the multiplication $\hat{y}=\hat{x}\cdot \hat{w} \in \mathbb{A}_{N,p}$ directly produces the 2-dimensional depth-wise convolution in certain coefficients of the resulting polynomial: 
\begin{align}
    \mathbf{Y}[k^{\prime}, g^{\prime}, i^{\prime},j^{\prime}]= \hat{y}[(\offset(k^\prime )+k')\times HWG^2  \\
    +\mathrm{O}-g^\prime HWG+i^{\prime} s W+j^{\prime} s]
\end{align}

\paragraph{Arithmetic Secret Sharing}
for ASS, an $l$-bit value $x$ is shared additively in
the ring $\mathbb{Z}_{2^l}$ as the sum of two values, say $\langle
x\rangle^S_{2^l}$ and  $\langle x\rangle^C_{2^l}$. To reconstruct the value
$x$, we compute the addition, i.e., $x\equiv \langle
x\rangle^S_{2^l}+\langle x\rangle^C_{2^l}$. In the two-party
setting, value $x\in \mathbb{Z}_{2^l}$ is secretly shared between the server and
client, by letting server hold the share $\langle x\rangle^S_{2^l}$ and letting
Bob hold another share $\langle x\rangle^C_{2^l}$\cite{huang2022cheetah}. 


\paragraph{Homomorphic Encryption}
this encryption scheme enables linearly homomorphic operations between ciphertexts and plaintext \cite{ElGamal_2007,Paillier_2007,hao2022iron}. HE encodes a 2D or 3D tensor into a 1D polynomial with two parameters: 
1) polynomial degree $N$ and 
2) ciphertext modulus $q$ and the bit width of each coefficient is $\log_2(q)$.


\begin{algorithm}[h]\label{alo:greedy packing}
\DontPrintSemicolon
  \SetAlgoLined
  Firstly, build a directed graph $G$ where vertices are the input strings $\{s_1,...,s_n\}$ , and the weight of the edge from string $s_i$ to string $s_j$ is the length of the longest suffix of $s_i$which is also a prefix of $s_j$. If there is no such overlap, there is no edge.\;
  
  Randomly select one of the longest edges\;
  
  Concatenate the nodes at both ends of the edge to form a new node. We define the merge of strings $s_i = \alpha \beta$ and $s_j = \beta \gamma$, where $\beta$ is the longest prefix-suffix overlap of $s_i$ and $s_j$, as the string $\alpha \beta \gamma$. Update the overlapping graph $G$\;
  
  Randomly select one of the longest edges on the new graph and perform step 3\;
  
  Repeat step 4 until there are no more edges in the graph. Concatenate the remaining nodes together to obtain the superstring $m$\;
  
  \caption{A greedy algorithm for SCS problem}
\end{algorithm}




We present the extended version of zero-aware greedy packing for group
convolution in Figure \ref{fig:pack_group}, we use $C_x^\prime$ and
$C_w^\prime$ to denote the number of groups that can be packed for input and
weight polynomials, respectively, with $C_x=C_x^\prime G^2$ and $C_w=C_w^\prime
G^2$.

\textbf{Complexity analysis}. Similar to Section \ref{subsec:greedy packing},
Cheetah achieves a coefficient utilization rate of $\frac{G}{C_x}$ in group
convolutions. As shown in Figure \ref{fig:pack_group}, when zero-aware greedy
packing is extended to group convolutions, we calculate that the theoretical
coefficient utilization rate is $\frac{C_w}{C_x+1+(C_w/2-1)(C_x+2)}$,
demonstrating that our method maintains the same approximate 2x improvement in
coefficient utilization even when extended to group convolutions. Moreover, it
brings about the same improvement in computational and communication
complexity.

\begin{figure}[!tbp]
\centerline{\includegraphics[width=1\linewidth]{figs/pack_group.pdf}}
\caption{\packmethod\ for group convolution. 
\ml{remove the figure. for group conv, no need to provide this many details and no need to have the complexity analysis.}}
\label{fig:pack_group}
\end{figure}

==> doc/outline.tex <==
\onecolumn

\section*{Outline}

\begin{itemize}
    \item Baseline methods:
    \begin{itemize}
        \item Cheetah,Iron,CrypTFlow2(HE) etc. (other OT works).
    \end{itemize}
    \item Motivation
    \begin{itemize}
        \item In the privacy-preserving inference framework based on MPC, the convolution operation is still one of the bottlenecks of communication and latency. In the plaintext domain, previous work proposed depth-wise convolution, which can reduce the amount of computation and parameters by number of channels times. More importantly, in modern state-of-the-art convolution neural networks such as ConvNeXt and lightweight networks such as MobileNetV2, depth-wise convolution is a ubiquitous operation. However, the existing state-of-the-art secure 2-party neural network inference framework like Cheetah, Iron can not fully enjoy the reduction of computation brought by depth-wise convolution, there is still high communication and latency and become one of the bottlenecks. Therefore, to design a new depth-wise convolution-friendly protocol is very important.
        \item Weakness of Cheetah and Iron
        \begin{itemize}
            \item Since Iron is designed for transformer networks, it only implements the matrix-matrix multiplication protocol. If it is necessary to perform depth-wise convolution operations, it can only be converted into C independent matrix-matrix multiplications, resulting in only one channel being encoded in a polynomial, which brings extremely big redundancy.
            \item Cheetah implements an efficient normal convolution protocol. To perform depth-wise separable convolution, a simple way is to execute the convolution protocol separately for each channel, which is essentially the same as Iron, and a polynomial can only encode one channel. Another way is to change the depth-wise separable convolution back to normal convolution by filling channels which are all zero, and then call the normal convolution protocol. In this process, the calculation of channels with all 0 values can be skipped, so that we can encode multiple channels or even multiple kernels into a polynomial. Unfortunately, there is a huge amount of waste in such encoding. It can be found that every C channels has C-1 channels that are all 0, resulting in a large number of 0 that need to be filled in the polynomial to complete a depth-wise convolution. The utilization rate of the polynomial coefficients is only 1/C.
        \end{itemize}
    \end{itemize}
    \item Key contributions: xxx
    \begin{itemize}
        \item Greedy Pack(GP): A novel depth-wise/group-wise encoding method which  enables to encode as many channels as possible into one polynomial by extremely reusing 0.
        \begin{itemize}
            \item depth-wise
            \item group-wise
        \end{itemize}
        \item Less Is More(LIM): A new tile strategy that intentionally reduces the number of channels encoded within one activation polynomial, allowing us to encode several times more kernels in a weight polynomial than before.
        \begin{itemize}
            \item The goal of previous tile strategies was all to fill a polynomial as much as possible, that is, to encode as many channels as possible. But we find that in depth-wise convolution, those strategies will lead to a large amount of zero waste in polynomials.
            Contrary to previous works, LIM intentionally reducing the number of activation channels encoded in a  polynomial, even if the polynomial can accommodate them. It enables us to encode much more weight channels in one polynomial.
        \end{itemize}
        \item With extensive experimental results, we demonstrate that for individual convolution, our proposed xxx reduces communication and latency by $ 2\sim 4$x compared to prior-art 2PC frameworks cheetah; for the whole networks, we reduce communication and latency by $1.2\sim 1.3$x compared to prior-art 2PC frameworks cheetah. 
    \end{itemize}
    \item Experimental results:
    \begin{itemize}
        \item Baselines: Cheetah, CrypTFlow2, Iron, (other OT works?), Ours, Ours+Tile Strategy
        \item Networks: MobileNetV2; Dataset: Cifar10/Cifar100
        \item Target: communication, latency, numOfPolyMul
        \item WAN: 9MB/s, refer to ABNN2, SecureML
        \item Micro-benchmark
            \begin{itemize}
                \item depth-wise conv under different dimensions
                \item group-wise conv under different group size
                \item depth-wise conv  under different N
                \item depth-wise conv under LAN/WAN(differnet bandwidth)  
            \end{itemize} 
        \item End-to-end Inference
            \begin{itemize}
                \item A whole network improvement is  about $1.2\sim1.3$ x
                \item We can expand channels by 1.2x to get higher accuracy but still a close latency.
            \end{itemize}
            
    \end{itemize}
\end{itemize}

Detailed outline:
\begin{itemize}
    \item 
\end{itemize}
